Deep Learning Models for Physical Layer Communications

The increased availability of data and computing resources has enabled researchers to successfully adopt machine learning (ML) techniques and make significant contributions in several engineering areas. ML and in particular deep learning (DL) algorithms have shown to perform better in tasks where a physical bottom-up description of the phenomenon is lacking and/or is mathematically intractable. Indeed, they take advantage of the observations of natural phenomena to automatically acquire knowledge and learn internal relations. Despite the historical model-based mindset, communications engineering recently started shifting the focus towards top-down data-driven learning models, especially in domains such as channel modeling and physical layer design, where in most of the cases no general optimal strategies are known. In this thesis, we aim at solving some fundamental open challenges in physical layer communications exploiting new DL paradigms. In particular, we mathematically formulate, under ML terms, classic problems such as channel capacity and optimal coding-decoding schemes, for any arbitrary communication medium. We design and develop the architecture, algorithm and code necessary to train the equivalent DL model, and finally, we propose novel solutions to long-standing problems in the field.

==> related_publications.tex <==
\section{Related publications}
\label{sec:relatedpub}
Below, we report the list of publications where the thesis main results have been documented. 

\noindent Journals:
\begin{itemize}
	\item A. M. Tonello, N. A. Letizia, D. Righini and F. Marcuzzi, "Machine Learning Tips and Tricks for Power Line Communications," in IEEE Access, vol. 7, pp. 82434-82452, June 2019, doi: 10.1109/ACCESS.2019.2923321.
     \item N. A. Letizia and A. M. Tonello, "Capacity-Driven Autoencoders for Communications," in IEEE Open Journal of the Communications Society, vol. 2, pp. 1366-1378, June 2021, doi: 10.1109/OJCOMS.2021.3087815.
	\item N. A. Letizia and A. M. Tonello, "Segmented Generative Networks: Data Generation in the Uniform Probability Space," in IEEE Transactions on Neural Networks and Learning Systems, vol. 33, no. 3, pp. 1338-1347, March 2022, doi: 10.1109/TNNLS.2020.3042380.
	
        \item A. M. Tonello and N. A. Letizia, "MIND: Maximum Mutual Information Based Neural Decoder," in IEEE Communications Letters, vol. 26, no. 12, pp. 2954-2958, Dec. 2022, doi: 10.1109/LCOMM.2022.3207379.
        \item N. A. Letizia, A. M. Tonello and H. Vincent Poor, "Cooperative Channel Capacity Learning," in IEEE Communications Letters, vol. 27, no. 8, pp. 1984-1988, Aug. 2023, doi: 10.1109/LCOMM.2023.3282307.
\end{itemize}
Conferences:
\begin{itemize}
	\item N. A. Letizia, A. M. Tonello and D. Righini, "Learning to Synthesize Noise: The Multiple Conductor Power Line Case," 2020 IEEE International Symposium on Power Line Communications and its Applications (ISPLC), Malaga, Spain, 2020, pp. 1-6, doi: 10.1109/ISPLC48789.2020.9115394.
	\item N. A. Letizia and A. M. Tonello, "Supervised Fault Detection in Energy Grids Measuring Electrical Quantities in the PLC Band," 2020 IEEE International Symposium on Power Line Communications and its Applications (ISPLC), Malaga, Spain, 2020, pp. 1-5, doi: 10.1109/ISPLC48789.2020.9115408.
	 10.1109/ISPLC48789.2020.9115397.
        \item N. A. Letizia and A. M. Tonello, "Capacity Learning for Communication Systems over Power Lines," 2021 IEEE International Symposium on Power Line Communications and its Applications (ISPLC), Aachen, Germany, 2021, pp. 55-60, doi: 10.1109/ISPLC52837.2021.9628415.
        \item N. A. Letizia and A. M. Tonello, "Discriminative Mutual Information Estimation for the Design of Channel Capacity Driven Autoencoders," 2022 International Balkan Conference on Communications and Networking (BalkanCom), Sarajevo, Bosnia and Herzegovina, 2022, pp. 41-45, doi: 10.1109/BalkanCom55633.2022.9900818.
        \item N. A. Letizia, N. Novello and A. M. Tonello, "Variational f-Divergence and Derangements for Discriminative Mutual Information Estimation", submitted to International Conference on Machine Learning 2024.
\end{itemize}
Other publications:
\begin{itemize}
    \item D. Righini, N. A. Letizia and A. M. Tonello, "Synthetic Power Line Communications Channel Generation with Autoencoders and GANs," 2019 IEEE International Conference on Communications, Control, and Computing Technologies for Smart Grids (SmartGridComm), Beijing, China, 2019, pp. 1-6, doi: 10.1109/SmartGridComm.2019.8909700.
     \item N. A. Letizia, B. Salamat and A. M. Tonello, "A New Recursive Framework for Trajectory Generation of UAVs," 2020 IEEE Aerospace Conference, Big Sky, MT, USA, 2020, pp. 1-8, doi: 10.1109/AERO47225.2020.9172656.
	\item F. Marcuzzi, A. M. Tonello and N. A. Letizia, "Discovering Routing Anomalies in Large PLC Metering Deployments from Field Data," 2020 IEEE International Symposium on Power Line Communications and its Applications (ISPLC), Malaga, Spain, 2020, pp. 1-6, doi:
         \item A. M. Tonello, N. A. Letizia and M. De Piante, "Learning the Impedance Entanglement for Wireline Data Communication," 2021 International Balkan Conference on Communications and Networking (BalkanCom), Novi Sad, Serbia, 2021, pp. 96-100, doi: 10.1109/BalkanCom53780.2021.9593164.
         
      \item N. A. Letizia, B. Salamat and A. M. Tonello, "A Novel Recursive Smooth Trajectory Generation Method for Unmanned Vehicles," in IEEE Transactions on Robotics, vol. 37, no. 5, pp. 1792-1805, Oct. 2021, doi: 10.1109/TRO.2021.3053649.
	\item B. Salamat, N. A. Letizia and A. M. Tonello, "Control Based Motion Planning Exploiting Calculus of Variations and Rational Functions: A Formal Approach," in IEEE Access, vol. 9, pp. 121716-121727, 2021, doi: 10.1109/ACCESS.2021.3109125.
	\item N. A. Letizia and A. M. Tonello, "Discriminative Mutual Information Estimators for Channel Capacity Learning", ArXiV 2107.03084.
     \item N. A. Letizia and A. M. Tonello, "Copula Density Neural Estimation," submitted to IEEE Transactions on Neural Networks.
\end{itemize}
